Locally Sparse Function on function Regression

In functional data analysis, functional linear regression has attracted significant attention recently. Herein, we consider the case where both the response and covariates are functions. There are two available approaches for addressing such a situation: concurrent and nonconcurrent functional models. In the former, the value of the functional response at a given domain point depends only on the value of the functional regressors evaluated at the same domain point, whereas, in the latter, the functional covariates evaluated at each point of their domain have a non-null effect on the response at any point of its domain. To balance these two extremes, we propose a locally sparse functional regression model in which the functional regression coefficient is allowed (but not forced) to be exactly zero for a subset of its domain. This is achieved using a suitable basis representation of the functional regression coefficient and exploiting an overlapping group-Lasso penalty for its estimation. We introduce efficient computational strategies based on majorization-minimization algorithms and discuss appealing theoretical properties regarding the model support and consistency of the proposed estimator. We further illustrate the empirical performance of the method through simulations and two applications related to human mortality and bidding the energy market.

==> 00_notation.tex <==
\newpage
\section*{ Open Issues}

{\color{red} MARCO = rosso}\\
{\color{teal} TONY = verde}\\
{\color{blue} MAURO = blu}


\begin{itemize}
    \item {\color{red} Nelle simu vinciamo anche contro ridge nello scenario pieno, come aggiustiamo?} \tony{No idea, andiamo di fine tuning con glmnet?}
    \item Dubbi sul numero di cose: Se abbiamo $M\times L$ coefficienti associati a spline di ordine $d$ dentro a $\Psib$, allora dovremmo avere (controllate please?)
    \begin{enumerate}
        \item $L-d+1$ nodi interni (verticali) e $M-d+1$ nodi interni (orizzontali)
        \item $L-d+3$ nodi totali (verticali) e $M-d+3$ nodi totali (orizzontali)
         \item $L-d+2 \times M-d+2$ quadratoni $\F_{m,l}$ e quindi nella Proposition 3 $m =1, \dots, M-d+2$
    \end{enumerate} 
\end{itemize}

==> 6_application_old.tex <==
\section{Application to basal body temperature functional time series}
\label{sec:app}

In this section we consider the analysis of the \citet{colombo2000daily} dataset and study the temporal evolution of basal body temperature (bbt) curves of  women
in their reproductive age. For woman $i$ data on $n_i$ menstrual cycles are available. Specifically, for each menstrual cycle $j$ with $j=1, \dots, n_i$ let  $y_{i,j}$ represent  the bbt curve with each $y_{i,j}: {\cal S} \to \R$ a smooth real function of the days within each menstrual cycle.
These  temperature curves typically show a characteristic  biphasic shape. Specifically, in the first phase of the cycle the curves are rather flat and constant. Then, around the ovulation, temperatures  rise to a higher value and remain constant for the last phase of the cycle. While such biphasic shape has been used as a clinical indicator of ovulation the lack of it may be an indicator fertility problem \citep{martinez1992reliability}. Previoius works used a FDA approach to analyze these data \citep{scarpa2009bayesian, canale2017pitman}  but to our knowledge none of them considered the possible temporal dependence of two consecutive cycles. Hence to fill this gap we introduce an autoregressive version of the locally sparse linear functional model defined in the previous sections. Specifically we let 
\[
y_{i,j} = \alpha_i + \Psib y_{i,j-1} + \epsilon_{i,j},
\]
where $\alpha_i$ is the woman specific intercept introduced to model the average level and shape of the functional data, $\Psib$ is the \HS autoregressive coefficient and $\epsilon_{i,j}$ is a functional random noise. It is interesting to induce a sparse structure in $\Psib$ in order to interpret the effect of this month's curve on the next one. Daily data are smoothed MARCO ? and centered on the. Figure \ref{fig:datibbt} reports a subsample of bbt curves for four random women in the study.

\begin{figure}
	\centering
	\includegraphics[width=0.7\textwidth]{img/fertili_4}
	\caption{Smoothed bbt data for 4 women}
	\label{fig:datibbt}
\end{figure}

==> tabellona.tex <==
% table
\begin{table}
\caption{Monte Carlo means and standard deviations ($\times 10^5$) of the $ISE_0$ and $ISE_1$ between the estimated coefficients  and the true coefficients $\psi_k$, $k=1,2,3,4$ over $100$ replicates.
Rows labelled S1 report the results for the default simulation settings, i.e. $n=50$, $SNR=4$, $L=M=20$; Rows labelled S2 report the results for $SNR =2$ and default remaining settings; 	Rows labelled S3 report the results for $L=M=40$ and default remaining settings; Rows labelled S4 report the results for $n = 150$ and default remaining settings.}
	\centering
	\resizebox{\textwidth}{!}{
	\begin{tabular}{crrrrrrrr}\toprule
		& Lasso & & Ridge  &  & LSFR &  & Enet & \\
		\cline{2-9}\\
		& \multicolumn{1}{c}{$ISE_0$} & 
		\multicolumn{1}{c}{\textit{$ISE_1$}} & 
		\multicolumn{1}{c}{$ISE_0$} & 
		\multicolumn{1}{c}{\textit{$ISE_1$}} & 
		\multicolumn{1}{c}{$ISE_0$} & 
		\multicolumn{1}{c}{\textit{$ISE_1$}} & 
		\multicolumn{1}{c}{$ISE_0$} &
		\multicolumn{1}{c}{\textit{$ISE_1$}} \\
		\cline{2-3}
		\cline{4-5}
		\cline{6-7}
		\cline{8-9}\\
		{\small $\psi_1$}\\
		\vspace*{.1cm}
		S1 &  0.18 \scriptsize{(0.06)}& 2.76
		\scriptsize{(0.44)}& 0.66 \scriptsize{(0.11)} & 1.12 \scriptsize{(0.22)}& 0.18 \scriptsize{(0.04)}& 1.07 \scriptsize{(0.20)}& 0.26 \scriptsize{(0.06)} & 1.34 \scriptsize{(0.23)}  \\
		\vspace*{.1cm}
		S2   & 0.31 \scriptsize{(0.12)}& 4.08 \scriptsize{(0.67)}& 0.98 \scriptsize{(0.17)}& 1.74 \scriptsize{(0.35)}& 0.28 \scriptsize{(0.08)}&  1.63 \scriptsize{(0.34)}& 0.42 \scriptsize{(0.12)} & 2.03 \scriptsize{(0.40)}   \\
		\vspace*{.1cm}
		 S3   & 0.37  \scriptsize{(0.13)}& 16.24 \scriptsize{(2.06)}& 1.02 \scriptsize{(0.20)}& 1.48 \scriptsize{(0.31)}& 0.14 \scriptsize{(0.05)}& 1.66 \scriptsize{(0.36)} & 0.39 \scriptsize{(0.11)} & 2.08 \scriptsize{(0.40)}  \\
		\vspace*{.1cm}
		S4   & 0.08  \scriptsize{(0.03)}& 1.45 \scriptsize{(0.24)}& 0.34 \scriptsize{(0.06)}& 0.56 \scriptsize{(0.09)}& 0.11 \scriptsize{(0.02)}& 0.58 \scriptsize{(0.09)} & 0.14 \scriptsize{(0.03)} & 0.71 \scriptsize{(0.11)}  \\
		\vspace*{.1cm}
		{\small $\psi_2$}\\
		\vspace*{.1cm}
		S1 &  0.12 \scriptsize{(0.07)}& 1.80 
		\scriptsize{(0.37)}& 0.52 \scriptsize{(0.14)} & 0.75 \scriptsize{(0.18)}& 0.04 \scriptsize{(0.03)}& 0.51 \scriptsize{(0.14)}& 0.16 \scriptsize{(0.08)} & 0.68 \scriptsize{(0.17)}  \\
		\vspace*{.1cm}
		S2   & 0.23  \scriptsize{(0.13)}& 2.42 \scriptsize{(0.47)}& 0.86 \scriptsize{(0.21)}& 1.21 \scriptsize{(0.26)}& 0.08 \scriptsize{(0.05)}&  0.82 \scriptsize{(0.22)}& 0.30 \scriptsize{(0.13)} & 1.09 \scriptsize{(0.25)}   \\
		\vspace*{.1cm}
		 S3   & 0.32  \scriptsize{(0.16)}& 9.98 \scriptsize{(2.75)}& 0.96 \scriptsize{(0.25)}& 1.16 \scriptsize{(0.26)}& 0.08 \scriptsize{(0.05)}& 0.74 \scriptsize{(0.21)} & 0.39 \scriptsize{(0.14)} & 1.04 \scriptsize{(0.23)}  \\
		\vspace*{.1cm}
		S4   & 0.04  \scriptsize{(0.02)}& 1.12 \scriptsize{(0.22)}& 0.26 \scriptsize{(0.07)}& 0.33 \scriptsize{(0.07)}& 0.02 \scriptsize{(0.01)}& 0.23 \scriptsize{(0.05)} & 0.06 \scriptsize{(0.03)} & 0.29 \scriptsize{(0.06)}  \\
		\vspace*{.1cm}
		{\small $\psi_3$}\\
		\vspace*{.1cm}
		S1 &  0.25 \scriptsize {(0.09)}& 1.01 \scriptsize{(0.19)} & 0.86 \scriptsize{(0.19)} & 1.10 \scriptsize{(0.16)} &  0.26 \scriptsize{(0.06)}& 0.58 \scriptsize{(0.11)} & 0.32 \scriptsize{(0.09)} & 0.69 \scriptsize{(0.11)}  \\
		\vspace*{.1cm}
		S2 & 0.32  \scriptsize{(0.15)}& 1.29 \scriptsize{(0.27)}& 1.14 \scriptsize{(0.30)}& 1.57 \scriptsize{(0.27)} & 0.32 \scriptsize{(0.09)}&  0.82 \scriptsize{(0.20)} & 0.40 \scriptsize{(0.15)} & 0.96 \scriptsize{(0.20)}   \\
		\vspace*{.1cm}
		 S3  & 0.47 \scriptsize{(0.14)}&  7.17 \scriptsize{(1.45)}& 1.18 \scriptsize{(0.29)}& 1.40 \scriptsize{(0.20)}& 0.25 \scriptsize{(0.07)}&  0.62 \scriptsize{(0.14)} & 0.41 \scriptsize{(0.12)} & 0.91 \scriptsize{(0.17)}  \\
		\vspace*{.1cm}
		S4   & 0.21  \scriptsize{(0.05)}&  0.68 \scriptsize{(0.13)}& 0.56 \scriptsize{(0.11)}& 0.61 \scriptsize{(0.09)}& 0.22 \scriptsize{(0.04)}& 0.36 \scriptsize{(0.06)} & 0.27 \scriptsize{(0.07)} & 0.46 \scriptsize{(0.08)}  \\
		\vspace*{.1cm}
		{\small $\psi_4$}\\
		\vspace*{.1cm}
		 S1 &  -- & 2.13 \scriptsize{(0.26)}& --  & 0.93 \scriptsize{(0.12)}& -- & 0.76 \scriptsize{(0.11)}& --  & 1.08 \scriptsize{(0.13)}  \\
		\vspace*{.1cm}
		 S2  & --  & 2.62 \scriptsize{(0.26)}& -- & 1.30   \scriptsize{(0.17)}& -- & 1.07 \scriptsize{(0.16)}& --  & 1.48 \scriptsize{(0.17)}   \\
		\vspace*{.1cm}
		 S3  & -- & 5.87 \scriptsize{(0.81)}& -- & 1.10 \scriptsize{(0.18)}& -- & 1.04 \scriptsize{(0.18)} & --  & 1.34 \scriptsize{(0.20)}  \\
		\vspace*{.1cm}
		 S4   & --  & 1.09 \scriptsize{(0.17)}& --& 0.53 \scriptsize{(0.06)}& -- & 0.42 \scriptsize{(0.06)} & --  & 0.61 \scriptsize{(0.08)}  \\
		\bottomrule
	\end{tabular}
	}
	\label{tab:tabellauno}
\end{table} 
